Scoring Strategic Agents

I introduce a model of predictive scoring. A receiver wants to predict a sender's quality. An intermediary observes multiple features of the sender and aggregates them into a score. Based on the score, the receiver makes a decision. The sender prefers "higher" decisions, and she can distort each feature at a privately known cost. I characterize the scoring rule that maximizes decision accuracy. This rule underweights some features to deter sender distortion, and overweights other features so that the score is correct on average. The receiver prefers this scoring rule to full disclosure because it mitigates his commitment problem.

==> feasible_scoring_asymmetric.tex <==
0.22857142857142865,-0.14395890252711602
0.22773785194484986,-0.14369071948372164
0.22487246253897386,-0.14285714285714285
0.21428571428571436,-0.1395874794169049
0.20621634857177748,-0.13664079428536544
0.20000000000000007,-0.13457574080411452
0.18650570227247576,-0.12936284512961854
0.18538786313772196,-0.12889785114799238
0.17142857142857149,-0.12248118991895711
0.16579374512432454,-0.1199205405899612
0.1571428571428572,-0.11592975479070802
0.15393471852689045,-0.11428571428571427
0.14675239601740464,-0.11039046112545253
0.1428571428571429,-0.10825963309511533
0.12964072219129666,-0.10106929361986802
0.12828535331429047,-0.1002860752571381
0.11428571428571432,-0.09157444421067398
0.11066469495317183,-0.0893353050468282
0.10521493703864523,-0.0857142857142857
0.09351242486574973,-0.07791614656282171
0.08571428571428574,-0.07235795327811567
0.07682044228009045,-0.06603670057705242
0.06510353718475544,-0.05714285714285713
0.06058048714400752,-0.05370522714170678
0.05714285714285717,-0.05109009457441515
0.04702605422572485,-0.042857142857142844
0.044784681500915316,-0.04092960421337041
0.042857142857142885,-0.039368784497759886
0.030361158129987745,-0.028571428571428553
0.029426054112504665,-0.027716803030352483
0.028571428571428595,-0.026935596179281922
0.014499046261381605,-0.014072382310046969
1.4772413277332487e-15,-1.4356079643098053e-15
2.0816681711721685e-17,-1.8562754339815623e-17
8.556195801443568e-19,8.556195801443568e-19
-1.8565360753533023e-17,2.0816681711721685e-17
-1.4356079643098055e-15,1.4772413277332489e-15
-0.014072366713252814,0.01449906185817576
-0.014285714285714266,0.014718915957550191
-0.026980955215299016,0.028571428571428595
-0.027716490531582975,0.029426366611274173
-0.028571428571428553,0.030421431397298446
-0.04092748850929547,0.04478679720499026
-0.05091688197113872,0.05714285714285717
-0.05369666584043533,0.060589048445278966
-0.05714285714285713,0.06514755625772212
-0.06601098909496626,0.0768461537621766
-0.07230351170568564,0.08571428571428574
-0.07785250495792412,0.09357606647064733
-0.0857142857142857,0.10553116381687809
-0.0891976802242962,0.11080231977570382
-0.09133786848072564,0.11428571428571432
-0.10001663345483468,0.12855479511659393
-0.10005924556462602,0.12863067413605464
-0.10770716272386349,0.1428571428571429
-0.10994834789615894,0.14719450924669822
-0.11428571428571427,0.15600165887017017
-0.11484192652980456,0.1571428571428572
-0.11532604227984845,0.1581831851369914
-0.11907059833237113,0.16664368738191462
-0.12107103472877372,0.17142857142857149
-0.12325354659468143,0.1767464534053186
-0.12554663276361425,0.18268948990647146
-0.12663263581855086,0.18571428571428578
-0.12713487533607948,0.18715083894963486
-0.12857142857142856,0.19157830296767234
-0.13065012695551612,0.1979213016159125
-0.13127999153201525,0.20000000000000007
-0.1335823670902672,0.20927477576687573
-0.13498523600717624,0.21428571428571436
-0.13659983093609748,0.22231411665038328
-0.13772789488508186,0.22857142857142865
-0.13837330046365143,0.23305527096492007
-0.13909039664606698,0.23909039664606707
-0.13937258051737658,0.24285714285714294
-0.13956187080061827,0.24615241491366752
-0.1398202821150441,0.2541059964007585
-0.13980939626669422,0.25714285714285723
-0.13964147707969093,0.26035852292030914
-0.13917688265314165,0.2677483112245703
-0.13873009183641066,0.2714285714285715
-0.1380310303305891,0.2762546839551253
-0.13736381756924218,0.28022096042638517
-0.1360673345291883,0.2857142857142858
-0.13450679831586623,0.29164965545872346
-0.13324739448249404,0.2953240340889346
-0.13154864802373206,0.3000000000000001
-0.13070713397012823,0.30213570539869977
-0.12857142857142856,0.3065175581284088
-0.12465937920882007,0.3142857142857144
-0.12072758115387379,0.3207275811538739
-0.11687737245882332,0.3259797703983196
-0.11496258410529274,0.3285714285714287
-0.11466214046402624,0.32894785474974064
-0.11428571428571427,0.32938094985246263
-0.10869041012461003,0.33571428571428585
-0.10792842071159157,0.3364998492830203
-0.10127515713199634,0.34285714285714297
-0.10060746678027974,0.3434646096374227
-0.09999999999999998,0.3439776630094984
-0.0941026371669739,0.348754505690169
-0.09272633479930553,0.3498691919421628
-0.0857142857142857,0.35465734790391573
-0.08193679223024733,0.35714285714285726
-0.0752357973239745,0.36095008303826037
-0.06038347835889023,0.3681879502125385
-0.05714285714285713,0.36976652239364904
-0.056011213582008265,0.3702969278677227
-0.053087616317429726,0.37142857142857155
-0.045632346059186375,0.37420377463061505
-0.042857142857142844,0.3750385353979743
-0.037399416176419925,0.37688629810929447
-0.03484251012421563,0.3776996529813586
-0.028571428571428553,0.37927368017545293
-0.0235710207239863,0.3807138778668436
-0.01803746782216878,0.3819625321778313
-0.014285714285714266,0.3827257152699602
-0.011874986528586944,0.38330355795715854
-0.00032063392804339286,0.3853936517862424
2.0816681711721685e-17,0.38544427107493784
0.0018667494111750844,0.38571428571428584
0.012859794563309069,0.3871402054366911
0.015991362359048328,0.38741993378761985
0.028571428571428595,0.3885435062330369
0.039446269252688654,0.3891251593187401
0.046386265699166825,0.3892434085563098
0.05714285714285717,0.38889182420508706
0.06790993734823277,0.38923291979462454
0.07460635315834417,0.3888920674440586
0.08571428571428574,0.3883236662598879
0.09847895962805153,0.38723532608623434
0.1012067549603247,0.38692104067461053
0.11428571428571432,0.38472012848176723
0.12626810487922674,0.38341096202208397
0.1317855678715598,0.3825001464141547
0.1428571428571429,0.3803479936692113
0.15010436893154647,0.3786757975029751
0.1684409649812544,0.3744161778758886
0.17142857142857149,0.37354572554520876
0.17313923670696932,0.37313923670696936
0.1789003973682493,0.37142857142857155
0.19496953317726043,0.36639810460583194
0.20000000000000007,0.3648113247057838
0.2102541982180207,0.3611743732105509
0.21610555903397727,0.3589627018911202
0.22857142857142865,0.35344022271485276
0.23616108574097963,0.3504468000266939
0.24285714285714294,0.34754600235482874
0.2527077761419579,0.34285714285714297
0.2556222943361516,0.3413365800504373
0.25714285714285723,0.3405884664225637
0.2620620892536885,0.3379379107463117
0.27408588709048853,0.3312287442333457
0.2857142857142858,0.32384434745753005
0.2917118990747235,0.3202833276461521
0.30055341760266313,0.3142857142857144
0.3086072772898369,0.3086072772898369
0.3142857142857144,0.3040882355271602
0.32472359616899066,0.2961521675975621
0.336836850465169,0.2857142857142858
0.3400227815680289,0.28287992442517174
0.34285714285714297,0.28004892973823803
0.3544787263617375,0.26876444064745175
0.3650895632864544,0.25714285714285723
0.36807841494254295,0.25379270065682863
0.37142857142857155,0.2495880308403464
0.3808224579499964,0.2379653150928535
0.3875646826149386,0.22857142857142865
0.3927249860473079,0.22129641461873636
0.40000000000000013,0.20981261622085512
0.4038129063545197,0.20381290635451962
0.4059616922167761,0.20000000000000007
0.4137059513998149,0.18629404860018528
0.41410529003891616,0.1855338614674875
0.42059192713466187,0.17142857142857149
0.42313237474900534,0.16598951760614808
0.4285714285714287,0.1527317805338985
0.4314220588348159,0.14570777312053004
0.43255397033374,0.1428571428571429
0.43464916279211097,0.13677940863646068
0.4385623602724844,0.12427664598677
0.4411923797657366,0.11428571428571432
0.44469640430716334,0.10183926145002038
0.4458372811293073,0.09701986172783571
0.44812230246104395,0.08571428571428574
0.44933660626102545,0.07790803483245388
0.45169617992877353,0.06258953435694092
0.4523229286927409,0.05714285714285717
0.45263242906361373,0.0526324290636136
0.45406073773168715,0.03165354798259873
0.45413472830876267,0.028571428571428595
0.45406314731406644,0.025491718742637733
0.45355266581100256,0.003590191331854734
0.4532884626732494,2.0816681711721685e-17
0.45274949789190005,-0.004393359250957242
0.4505866183803376,-0.022015189808908875
0.44940155736117354,-0.028571428571428553
0.4470514985794931,-0.038662787134792716
0.44546450552146494,-0.04546450552146476
0.442857142857143,-0.054121790651744175
0.44186119998420037,-0.05714285714285713
0.4381215847015842,-0.06669301327301261
0.4292878727346342,-0.0849978415510802
0.42894140116041063,-0.0857142857142857
0.4288138675969439,-0.08595672473980087
0.4285714285714287,-0.08636711425110194
0.42453056445342496,-0.09285714285714283
0.42329610072468066,-0.09472467215325192
0.4214285714285716,-0.09742960944171497
0.4195521120122391,-0.09999999999999998
0.41725779488879283,-0.1029720806030784
0.4142857142857144,-0.10648596158757027
0.40707121878447894,-0.11428571428571427
0.40355704043510904,-0.11784275472082319
0.40000000000000013,-0.12091732636905238
0.390180277539909,-0.12857142857142856
0.38760446126060066,-0.13046160411774335
0.38571428571428584,-0.13163610628116507
0.3787595679515864,-0.1359024250944434
0.377982122354256,-0.13630359193145838
0.37142857142857155,-0.13959621078265136
0.3692486017148586,-0.14067717314342995
0.3639203841759154,-0.14285714285714285
0.35714285714285726,-0.14548837427787922
0.3482064405375531,-0.14820644053755302
0.34285714285714297,-0.14962763660635794
0.3367920048402399,-0.15107771912595408
0.3341747073361587,-0.15153957837812712
0.3285714285714287,-0.15242201768941424
0.32448746103518494,-0.15305888960661343
0.3176934066481444,-0.15373516478042712
0.3142857142857144,-0.1540068260050976
0.3113792601329633,-0.15423640299010602
0.30266145550400864,-0.15448140163884863
0.3000000000000001,-0.15454644325867523
0.29737894159253964,-0.15452179873539668
0.28866913894059326,-0.15418800391654966
0.2857142857142858,-0.15401292840139902
0.2823895765111609,-0.15381814793973222
0.2754485963563355,-0.15312283221509315
0.2714285714285715,-0.1526346739386271
0.2661914180958158,-0.15190570381010146
0.25714285714285723,-0.1504509731988477
0.25092274755826044,-0.1490772524417396
0.23007348521828075,-0.14435919950399495
0.22857142857142865,-0.14395890252711602


==> feasible_scoring_symmetric.tex <==
0.22857142857142865,-0.14507807888169474
0.2269053338052639,-0.1445232376233076
0.22136788380686034,-0.14285714285714285
0.21428571428571436,-0.1406113341381818
0.2055290291814065,-0.1373281136757364
0.20000000000000007,-0.13544346554444195
0.18771792695728795,-0.13057506981443073
0.18490834392178146,-0.12937737036393288
0.17142857142857149,-0.12309421218778062
0.1654281723123974,-0.12028611340188836
0.1571428571428572,-0.11639405552581318
0.15310260016672161,-0.11428571428571427
0.14649059144885013,-0.11065226569400705
0.1428571428571429,-0.10865127364814542
0.13027156615962576,-0.10170013758819713
0.12812623480387994,-0.10044519376754865
0.11428571428571432,-0.0917732426303855
0.1105617292419323,-0.08943827075806772
0.10500390794615717,-0.0857142857142857
0.09345170059318614,-0.0779768708353853
0.08571428571428574,-0.07244863831820356
0.07678872358941474,-0.06606841926772812
0.06506486181613083,-0.05714285714285713
0.06056652220032811,-0.05371919208538618
0.05714285714285717,-0.051111013122957044
0.04701462094924423,-0.042857142857142844
0.04477996618379565,-0.04093431953049008
0.042857142857142885,-0.039376480853050164
0.030358971087757328,-0.028571428571428553
0.02942506826811145,-0.0277177888747457
0.028571428571428595,-0.02693748084176298
0.014498981963411603,-0.01407244660801697
1.47768708104258e-15,-1.4360537176191366e-15
2.0816681711721685e-17,-1.8565360753533023e-17
8.555358744985878e-19,8.555358744985878e-19
-1.8565360753533023e-17,2.0816681711721685e-17
-1.4360537176191366e-15,1.47768708104258e-15
-0.01407244660801697,0.014498981963411603
-0.014285714285714266,0.014718723149540884
-0.026982898767261697,0.028571428571428595
-0.0277177888747457,0.02942506826811145
-0.028571428571428553,0.030416980279993955
-0.04093431953049008,0.04477996618379565
-0.05094712962379484,0.05714285714285717
-0.05371919208538618,0.06056652220032811
-0.05714285714285713,0.06506486181613083
-0.06606841926772812,0.07678872358941474
-0.07244863831820356,0.08571428571428574
-0.0779768708353853,0.09345170059318614
-0.0857142857142857,0.10500390794615717
-0.08943827075806772,0.1105617292419323
-0.0917732426303855,0.11428571428571432
-0.10044519376754865,0.12812623480387994
-0.10170013758819713,0.13027156615962576
-0.10879575015467016,0.1428571428571429
-0.11065226569400705,0.14649059144885013
-0.11428571428571427,0.15310260016672161
-0.11639405552581318,0.1571428571428572
-0.12028611340188836,0.1654281723123974
-0.12309421218778062,0.17142857142857149
-0.12937737036393288,0.18490834392178146
-0.13057506981443073,0.18771792695728795
-0.13544346554444195,0.20000000000000007
-0.1373281136757364,0.2055290291814065
-0.14285714285714285,0.22196985268927716
-0.1445232376233076,0.2269053338052639
-0.14502065837337766,0.22857142857142865
-0.14592411550486378,0.23163840121914958
-0.15018901243085833,0.24981098756914175
-0.15186806133626243,0.25714285714285723
-0.15268516899003026,0.26160054529568405
-0.15373856008827044,0.2680242743739848
-0.15417236715321625,0.2714285714285715
-0.1544985020706098,0.2740729265008188
-0.15554475552077826,0.28411618409220696
-0.1556464663299078,0.2857142857142858
-0.15572954242421355,0.2871276004329294
-0.15620569556047198,0.29906283841761494
-0.1562009166270459,0.3000000000000001
-0.15619062505030512,0.3009522320925521
-0.15583833876360284,0.3129811959064601
-0.15573488289292473,0.3142857142857144
-0.15560249907448756,0.31582607235408394
-0.15454835495841002,0.32597692638698156
-0.15413443528618154,0.3285714285714287
-0.15353045490347314,0.3321838308108127
-0.15243152598210882,0.3381458116963947
-0.15127053306860433,0.34285714285714297
-0.14944398561904526,0.3494439856190454
-0.14699662403599292,0.35714285714285726
-0.14285714285714285,0.36734481888735543
-0.1416400163673846,0.3702114449388133
-0.1410512492843983,0.37142857142857155
-0.13899265173104636,0.37529306255466804
-0.13670421199056806,0.37956135484771103
-0.13280311553809057,0.38571428571428584
-0.13113870009528078,0.38828155723813806
-0.12857142857142856,0.3918838862041364
-0.12784901210762498,0.392857142857143
-0.12499517591818349,0.39642374734675506
-0.12200368717216387,0.40000000000000013
-0.12142857142857141,0.4006417063365541
-0.11828602688947745,0.4040003126037633
-0.11521471302633007,0.40714285714285725
-0.11428571428571427,0.40803458909357043
-0.11102472748189027,0.4110247274818904
-0.1073112056989254,0.4142857142857144
-0.10714285714285712,0.41442500463096343
-0.10322572443549698,0.41751143872121144
-0.09999999999999998,0.4197873154140629
-0.094904321599984,0.42347575017141276
-0.08667232713766602,0.4285714285714287
-0.08607656554821944,0.42893370840536243
-0.0857142857142857,0.4291208489430905
-0.08453552917667524,0.4297501851090392
-0.07669771090693196,0.43384056804978927
-0.07142857142857141,0.43614889092793774
-0.06674016565412733,0.43816873708269893
-0.05714285714285713,0.44129282962314575
-0.0454748429495881,0.4454748429495883
-0.03865368692831936,0.4470605987859665
-0.028571428571428553,0.4494033625612781
-0.022016060956458097,0.45058748952788685
-0.004393321642375946,0.4527495355004813
2.0816681711721685e-17,0.45313216354770136
0.0035901662170744163,0.4535526909257829
0.025493055579795178,0.45406448415122386
0.028571428571428595,0.4541363646435772
0.031650403410221836,0.454063882304064
0.05265080348180516,0.4526508034818053
0.05714285714285717,0.45217151717170617
0.06254586235166093,0.4517398519340535
0.07798353608569585,0.4494121075142674
0.08571428571428574,0.44793056444784074
0.096767738563104,0.44608940429403904
0.10203037857690102,0.444887521434044
0.11428571428571432,0.4415721059475602
0.12470923678341118,0.43899495106912556
0.1356211677597515,0.43580740366882015
0.1428571428571429,0.4333146765579198
0.1464422283636728,0.4321565140779586
0.15701534483628213,0.4285714285714287
0.1571428571428572,0.4285252431624922
0.16724582933295248,0.42438868647580974
0.17142857142857149,0.42280293781065426
0.18147720406586804,0.41852279593413216
0.18731824218712834,0.415889670758557
0.20000000000000007,0.4095387075468418
0.218372949447606,0.40000000000000013
0.22496809442276564,0.39639666585133715
0.22857142857142865,0.39422286039392046
0.24265585654015445,0.3859155720312743
0.2429041025176773,0.3857612453748202
0.25714285714285723,0.37607725366333555
0.25992799074000467,0.374213705025719
0.26398905736542705,0.37142857142857155
0.2714285714285715,0.36598102850609854
0.27636413243659874,0.3620784181508845
0.2829550331724734,0.35714285714285726
0.2857142857142858,0.3549337673898633
0.29219714766905763,0.3493400048119148
0.29960175923194493,0.34285714285714297
0.30741580522920153,0.3359872338006301
0.3142857142857144,0.32940547844245166
0.32201326613290854,0.32201326613290854
0.32940547844245166,0.3142857142857144
0.3359872338006301,0.30741580522920153
0.34285714285714297,0.29960175923194493
0.3493400048119148,0.29219714766905763
0.35453029022259785,0.2857142857142858
0.3620784181508845,0.27636413243659874
0.37142857142857155,0.2637262234736825
0.374213705025719,0.25992799074000467
0.376231478958358,0.25714285714285723
0.38571428571428584,0.24297889766453493
0.3857612453748202,0.2429041025176773
0.3859155720312743,0.24265585654015445
0.39422286039392046,0.22857142857142865
0.39639666585133715,0.22496809442276564
0.40000000000000013,0.218372949447606
0.4064277912958945,0.20642779129589445
0.4095387075468418,0.20000000000000007
0.415889670758557,0.18731824218712834
0.41852279593413216,0.18147720406586804
0.42260858740417234,0.17142857142857149
0.42438868647580974,0.16724582933295248
0.4285714285714287,0.15614865224094812
0.4321565140779586,0.1464422283636728
0.433473018432735,0.1428571428571429
0.43580740366882015,0.1356211677597515
0.43899495106912556,0.12470923678341118
0.4415721059475602,0.11428571428571432
0.444887521434044,0.10203037857690102
0.44608940429403904,0.096767738563104
0.4482435075916871,0.08571428571428574
0.4494121075142674,0.07798353608569585
0.4517398519340535,0.06254586235166093
0.4523479402133469,0.05714285714285717
0.4526508034818053,0.05265080348180516
0.454063882304064,0.031650403410221836
0.4541363646435772,0.028571428571428595
0.45406448415122386,0.025493055579795178
0.4535526909257829,0.0035901662170744163
0.4532884626732494,2.0816681711721685e-17
0.4527495355004813,-0.004393321642375946
0.45058748952788685,-0.022016060956458097
0.4494033625612781,-0.028571428571428553
0.4470605987859665,-0.03865368692831936
0.4454748429495883,-0.0454748429495881
0.442857142857143,-0.05420871233420385
0.4418945355312224,-0.05714285714285713
0.43816873708269893,-0.06674016565412733
0.42962213689924533,-0.08466357738646905
0.4291208489430905,-0.0857142857142857
0.42893370840536243,-0.08607656554821944
0.4285714285714287,-0.0867002492552108
0.4248021106590641,-0.09285714285714283
0.42347575017141276,-0.094904321599984
0.4214285714285716,-0.09792792809959018
0.41994514794265564,-0.09999999999999998
0.41751143872121144,-0.10322572443549698
0.4142857142857144,-0.1071408261128494
0.40783502975866737,-0.11428571428571427
0.4040003126037633,-0.11828602688947745
0.40000000000000013,-0.12186228514926464
0.3916523384476163,-0.12857142857142856
0.38828155723813806,-0.13113870009528078
0.38571428571428584,-0.13280311553809057
0.37956135484771103,-0.13670421199056806
0.37529306255466804,-0.13899265173104636
0.37142857142857155,-0.14101763971220732
0.3702114449388133,-0.1416400163673846
0.36734481888735543,-0.14285714285714285
0.35714285714285726,-0.14699662403599292
0.3494439856190454,-0.14944398561904526
0.34285714285714297,-0.15127053306860433
0.3381458116963947,-0.15243152598210882
0.3321838308108127,-0.15353045490347314
0.3285714285714287,-0.15413443528618154
0.32597692638698156,-0.15454835495841002
0.31582607235408394,-0.15560249907448756
0.3142857142857144,-0.15573488289292473
0.3129811959064601,-0.15583833876360284
0.3009522320925521,-0.15619062505030512
0.3000000000000001,-0.15621487969252298
0.29906283841761494,-0.15620569556047198
0.2871276004329294,-0.15572954242421355
0.2857142857142858,-0.1556464663299078
0.28411618409220696,-0.15554475552077826
0.2740729265008188,-0.1544985020706098
0.2714285714285715,-0.15417236715321625
0.26795646982542654,-0.15367075553971216
0.25714285714285723,-0.15186806133626243
0.24981098756914175,-0.15018901243085833
0.23163840121914958,-0.14592411550486378
0.22857142857142865,-0.14507807888169474


==> scoring_1.tex <==
1.0000000612244897,0.32218534904303003
1.0009201537616788,0.3221996560169892
1.001840246298868,0.3222139368281697
1.0036804313732461,0.3222425317897876
1.0073608015220024,0.32229954612574424
1.0147215418195152,0.3224135167753403
1.0294430224145406,0.3226400589407396
1.0588859836045912,0.3230884822510772
1.122725071256376,0.3240390885216646
1.1823336507104565,0.32490170010770525
1.2407729464566284,0.3257250585016626
1.3041654074744837,0.32659405014082526
1.3633273602946345,0.3273846621940916
1.4274424783864688,0.32821763907642815
1.4903883127703945,0.32901483649249696
1.549103638956616,0.32974077126775575
1.6127721304145206,0.33050822688980247
1.672210113674721,0.3312075110447621
1.7304788132270128,0.3318807832685002
1.7937006780509879,0.33259120414711235
1.8526920346772586,0.33324046608789226
1.9166365565752128,0.3339284747851128
1.9794117947652585,0.3345885632299384
2.0379565247576,0.33519119436497224
2.101454420021624,0.3358312215358116
2.160721807087944,0.33641626515463424
2.2249423594259476,0.33703743482967274
2.2879936280560424,0.337634618623152
2.3468143884884327,0.33818101140955814
2.4105883141925064,0.33876184089226097
2.4701317316988756,0.33929388082528894
2.5285058654973365,0.3398062172915797
2.591833164567481,0.3403517706159105
2.6509299554399206,0.3408516572334819
2.714979911584044,0.3413837296705043
2.7778605840202584,0.34189652853639324
2.836510748258769,0.342366639474569
2.9001140777689622,0.34286770345548917
2.9594868990814516,0.34332756926331
3.017690436686032,0.34377113243336077
3.0808471395622963,0.34424460812541274
3.139773334240856,0.3446782844432925
3.2036526941910988,0.345142466281235
3.263301545943637,0.34556879899191423
3.3217811139882674,0.34598018344050446
3.385213847304581,0.3464189784017798
3.44441607242319,0.34682285379149724
3.5085714628134825,0.3472555019963361
3.5715575694958663,0.3476719198248457
3.630313167980546,0.34805428115692005
3.694021931736909,0.34846009944908574
3.753500187295568,0.3488364586693572
3.8118091591463177,0.34920230871129515
3.875071296268751,0.34959176831212563
3.93410292519348,0.3499499600236071
3.935132566030699,0.34995616656094947
3.936162206867918,0.34996237224371307
3.9382214885423563,0.34997477805624816
3.9423400518912333,0.34999969595595226
3.950577178588987,0.3500491633050651
3.967051431984495,0.3501478702658712
3.968081072821714,0.35015403427443087
3.9691107136589334,0.35016070232849333
3.971169995333372,0.35017301269204276
3.975288558682249,0.35019753356238875
3.9835256853800027,0.35024683504650855
3.984555326217222,0.35025297228508684
3.985584967054441,0.350259072389244
3.9876442487288797,0.3502713850737154
3.9917628120777566,0.3502958803286801
3.992792452914976,0.35030196018286835
3.993822093752195,0.3503080908210352
3.9958813754266336,0.35032014003887046
3.996911016263853,0.35032646158783703
3.997940657101072,0.3503323832323224
3.998970297938291,0.3503384989953374
3.99999993877551,0.35034461418940616


==> scoring_2.tex <==
1.0000000612244897,0.32218534863762216
1.0009201537616788,0.3221617532019154
1.001840246298868,0.3221381816378326
1.0036804313732461,0.3220910193114732
1.0073608015220024,0.3219969057345946
1.0147215418195152,0.3218088781219949
1.0294430224145406,0.32143478465595915
1.0588859836045912,0.32069348475440734
1.122725071256376,0.31911777898840726
1.1823336507104565,0.3176833380064735
1.2407729464566284,0.3163100265946934
1.3041654074744837,0.3148559369701718
1.3633273602946345,0.31352962688862535
1.4274424783864688,0.31212695275967584
1.4903883127703945,0.31078101346487
1.549103638956616,0.3095523056815547
1.6127721304145206,0.3082492200475741
1.672210113674721,0.30705855992485753
1.7304788132270128,0.30591142094012697
1.7937006780509879,0.3046953425809365
1.8526920346772586,0.30358197088845146
1.9166365565752128,0.30239901345625797
1.9794117947652585,0.30126098794948675
2.0379565247576,0.30021950955899396
2.101454420021624,0.29911078040495087
2.160721807087944,0.29809488348100865
2.2249423594259476,0.29701385723149776
2.2879936280560424,0.2959720613078338
2.3468143884884327,0.2950168506185002
2.4105883141925064,0.2939990793885668
2.4701317316988756,0.29306484797175514
2.5285058654973365,0.29216347466005865
2.591833164567481,0.29120159296947745
2.6509299554399206,0.2903184199802626
2.714979911584044,0.2893764840707914
2.7778605840202584,0.2884667690736804
2.836510748258769,0.2876311983580519
2.9001140777689622,0.28673886188964154
2.9594868990814516,0.28591837326811115
3.017690436686032,0.28512552091706156
3.0808471395622963,0.2842776542732968
3.139773334240856,0.2834989000549942
3.2036526941910988,0.2826651437450607
3.263301545943637,0.28189784284867414
3.3217811139882674,0.28115596337808557
3.385213847304581,0.28036282367275694
3.44441607242319,0.2796320387362068
3.5085714628134825,0.27884917692730304
3.5715575694958663,0.27809293634772936
3.630313167980546,0.27739707420859383
3.694021931736909,0.2766550580993988
3.753500187295568,0.2759682555471644
3.8118091591463177,0.27530120629689886
3.875071296268751,0.27458842541841655
3.93410292519348,0.27393170480428974
3.935132566030699,0.27392031783759746
3.936162206867918,0.2739089326735829
3.9382214885423563,0.2738861707225609
3.9423400518912333,0.27384055189241957
3.950577178588987,0.2737497267594681
3.967051431984495,0.2735684811074511
3.968081072821714,0.2735571661854667
3.9691107136589334,0.2735453477099555
3.971169995333372,0.2735227395246487
3.975288558682249,0.2734776323144137
3.9835256853800027,0.2733872045993441
3.984555326217222,0.273375930625491
3.985584967054441,0.2733646936234871
3.9876442487288797,0.27334211328397046
3.9917628120777566,0.27329708949201925
3.992792452914976,0.27328588290792677
3.993822093752195,0.2732746219257458
3.9958813754266336,0.27325232002294864
3.996911016263853,0.2732408716414602
3.997940657101072,0.27322982489130637
3.998970297938291,0.27321858428846757
3.99999993877551,0.2732073450816721


==> scoring_BR_1.tex <==
1.0000000612244897,0.32218535557262085
1.0009201537616788,0.32219108191619744
1.001840246298868,0.32219680966889497
1.0036804313732461,0.32220824964266664
1.0073608015220024,0.32223112441521207
1.0147215418195152,0.3222767323738814
1.0294430224145406,0.3223676062532226
1.0588859836045912,0.3225478432193315
1.122725071256376,0.32293209781239574
1.1823336507104565,0.3232829898621495
1.2407729464566284,0.32361993158830094
1.3041654074744837,0.3239779328284007
1.3633273602946345,0.3243050481124802
1.4274424783864688,0.32465279788322154
1.4903883127703945,0.32498715500648484
1.549103638956616,0.32529301910821284
1.6127721304145206,0.3256186516060826
1.672210113674721,0.3259170773592327
1.7304788132270128,0.32620389353057117
1.7937006780509879,0.32651044140885904
1.8526920346772586,0.32679126204785114
1.9166365565752128,0.3270905215150206
1.9794117947652585,0.3273792939188842
2.0379565247576,0.3276442368930092
2.101454420021624,0.32792698204803167
2.160721807087944,0.3281867098482735
2.2249423594259476,0.32846369320918717
2.2879936280560424,0.32873132903155505
2.3468143884884327,0.32897723516959093
2.4105883141925064,0.32923993192566003
2.4701317316988756,0.3294815745796777
2.5285058654973365,0.32971515949899244
2.591833164567481,0.3299650203806062
2.6509299554399206,0.33019493220793245
2.714979911584044,0.3304406609752358
2.7778605840202584,0.3306785205906938
2.836510748258769,0.3308974183439006
2.9001140777689622,0.33113168744310983
2.9594868990814516,0.3313474996843369
3.017690436686032,0.3315564611844662
3.0808471395622963,0.33178035458662186
3.139773334240856,0.3319869019940595
3.2036526941910988,0.3322075934092217
3.263301545943637,0.3324111844844151
3.3217811139882674,0.3326085451515766
3.385213847304581,0.3328202494320256
3.44441607242319,0.3330153373240041
3.5085714628134825,0.333223805481588
3.5715575694958663,0.33342654823721873
3.630313167980546,0.3336136597715592
3.694021931736909,0.3338150790823277
3.753500187295568,0.33400015888051854
3.8118091591463177,0.3341791117885398
3.875071296268751,0.33437174986875057
3.93410292519348,0.3345496331551206
3.935132566030699,0.3345527191222752
3.936162206867918,0.3345558043645164
3.9382214885423563,0.3345619735703178
3.9423400518912333,0.33457426828407877
3.950577178588987,0.3345989212148986
3.967051431984495,0.33464810767119135
3.968081072821714,0.3346511750777567
3.9691107136589334,0.33465408962520554
3.971169995333372,0.3346602247635191
3.975288558682249,0.3346725131851522
3.9835256853800027,0.3346969655343307
3.984555326217222,0.33470002537314736
3.985584967054441,0.3347030952699373
3.9876442487288797,0.33470919878417865
3.9917628120777566,0.3347214327801454
3.992792452914976,0.3347245026416499
3.993822093752195,0.3347275554724687
3.9958813754266336,0.33473372312269045
3.996911016263853,0.33473671554238754
3.997940657101072,0.3347398278856905
3.998970297938291,0.3347428805440688
3.99999993877551,0.3347459323971189


==> scoring_BR_2.tex <==
1.0000000612244897,0.3221853537938417
1.0009201537616788,0.32217033634890374
1.001840246298868,0.322155321134187
1.0036804313732461,0.32212531574709474
1.0073608015220024,0.3220653494859089
1.0147215418195152,0.3219457155828826
1.0294430224145406,0.32170741327173213
1.0588859836045912,0.3212347804163711
1.122725071256376,0.3202275043178231
1.1823336507104565,0.3193079074916751
1.2407729464566284,0.31842509322044565
1.3041654074744837,0.3174874578664735
1.3633273602946345,0.3166306561786719
1.4274424783864688,0.315720591167715
1.4903883127703945,0.31484558261191437
1.549103638956616,0.3140451848391379
1.6127721304145206,0.31319351934038786
1.672210113674721,0.3124132583524014
1.7304788132270128,0.31166253261288973
1.7937006780509879,0.31086154137258487
1.8526920346772586,0.31012756499463157
1.9166365565752128,0.30934567308533334
1.9794117947652585,0.30859146172246155
2.0379565247576,0.3078996684512227
2.101454420021624,0.3071615751895886
2.160721807087944,0.3064837529126152
2.2249423594259476,0.3057610324551098
2.2879936280560424,0.3050629120148049
2.3468143884884327,0.30442158875117914
2.4105883141925064,0.30373669824658944
2.4701317316988756,0.30310682075342427
2.5285058654973365,0.3024980434882526
2.591833164567481,0.30184703309312627
2.6509299554399206,0.3012481371502132
2.714979911584044,0.3006081813715658
2.7778605840202584,0.29998887639659255
2.836510748258769,0.29941905027427257
2.9001140777689622,0.29880935942072095
2.9594868990814516,0.29824780515696886
3.017690436686032,0.2977042020473813
3.0808471395622963,0.2971218754895732
3.139773334240856,0.2965851163332813
3.2036526941910988,0.29601114105082826
3.263301545943637,0.2954818204009807
3.3217811139882674,0.2949689060555269
3.385213847304581,0.2944190381393508
3.44441607242319,0.2939122118785048
3.5085714628134825,0.29337013538213425
3.5715575694958663,0.2928437148246231
3.630313167980546,0.2923581270018827
3.694021931736909,0.2918365324910909
3.753500187295568,0.29135624668969856
3.8118091591463177,0.290891222823287
3.875071296268751,0.2903914559801632
3.93410292519348,0.28993012138956614
3.935132566030699,0.28992211823752717
3.936162206867918,0.2899141167716235
3.9382214885423563,0.28989811769646534
3.9423400518912333,0.2898661867747323
3.950577178588987,0.28980227392045516
3.967051431984495,0.28967474499735135
3.968081072821714,0.2896667895316826
3.9691107136589334,0.2896590403439698
3.971169995333372,0.28964313259543106
3.975288558682249,0.28961130136812335
3.9835256853800027,0.2895478398023824
3.984555326217222,0.28953990584520817
3.985584967054441,0.289531959193382
3.9876442487288797,0.28951611637288616
3.9917628120777566,0.28948440337961406
3.992792452914976,0.28947646119251447
3.993822093752195,0.2894685431961891
3.9958813754266336,0.2894526251983569
3.996911016263853,0.28944479051022703
3.997940657101072,0.2894367949968442
3.998970297938291,0.2894288805997169
3.99999993877551,0.28942096799433814


==> screening_1.tex <==
1.0000000612244897,0.31290841013797227
1.0009201537616788,0.3129183022157453
1.001840246298868,0.31292820022834905
1.0036804313732461,0.3129479624011257
1.0073608015220024,0.31298746049835374
1.0147215418195152,0.3130662187317834
1.0294430224145406,0.3132228670289528
1.0588859836045912,0.31353274722824775
1.122725071256376,0.31418951153678165
1.1823336507104565,0.3147849175418626
1.2407729464566284,0.3153528122297163
1.3041654074744837,0.31595203129611854
1.3633273602946345,0.31649627409744885
1.4274424783864688,0.3170705695746914
1.4903883127703945,0.3176194661080073
1.549103638956616,0.31811878176835984
1.6127721304145206,0.3186470186819654
1.672210113674721,0.3191283196861811
1.7304788132270128,0.3195895419271975
1.7937006780509879,0.32007859572523123
1.8526920346772586,0.3205246932633194
1.9166365565752128,0.32099756172776284
1.9794117947652585,0.3214514161600855
2.0379565247576,0.3218658015483186
2.101454420021624,0.32230593612814523
2.160721807087944,0.32270833751900513
2.2249423594259476,0.3231355505848123
2.2879936280560424,0.32354641550719543
2.3468143884884327,0.323922323234869
2.4105883141925064,0.3243221236212897
2.4701317316988756,0.32468836756333747
2.5285058654973365,0.32504105005147715
2.591833164567481,0.3254167662947359
2.6509299554399206,0.32576112668336527
2.714979911584044,0.3261277566043092
2.7778605840202584,0.326481241066411
2.836510748258769,0.32680536738152494
2.9001140777689622,0.32715097659879055
2.9594868990814516,0.3274682362610013
3.017690436686032,0.32777437389267106
3.0808471395622963,0.328101266778075
3.139773334240856,0.3284014356531627
3.2036526941910988,0.32872172847857156
3.263301545943637,0.32901614898701753
3.3217811139882674,0.3293005517860432
3.385213847304581,0.3296044229878309
3.44441607242319,0.3298838079336997
3.5085714628134825,0.3301820957245662
3.5715575694958663,0.3304705457395933
3.630313167980546,0.33073579657310614
3.694021931736909,0.33101934685513407
3.753500187295568,0.3312803522982724
3.8118091591463177,0.33153283175478493
3.875071296268751,0.3318030520074788
3.93410292519348,0.33205180843452814
3.935132566030699,0.33205611870973273
3.936162206867918,0.3320604280131151
3.9382214885423563,0.33206904370604545
3.9423400518912333,0.33208626344795916
3.950577178588987,0.33212065644690875
3.967051431984495,0.3321892572292236
3.968081072821714,0.3321935352740266
3.9691107136589334,0.33219781502578133
3.971169995333372,0.33220636898829825
3.975288558682249,0.33222346542397374
3.9835256853800027,0.3322576124270281
3.984555326217222,0.33226187650999894
3.985584967054441,0.3322661396404212
3.9876442487288797,0.3322746630452018
3.9917628120777566,0.33229169844156636
3.992792452914976,0.3322959549152089
3.993822093752195,0.33230021043946045
3.9958813754266336,0.33230871864136347
3.996911016263853,0.3323129713198013
3.997940657101072,0.33231722305042116
3.998970297938291,0.3323214738336142
3.99999993877551,0.3323257236697742


==> screening_2.tex <==
1.0000000612244897,0.3129084077747671
1.0009201537616788,0.3128827934217256
1.001840246298868,0.3128572007735371
1.0036804313732461,0.3128060434380052
1.0073608015220024,0.3127038556026225
1.0147215418195152,0.31250003600336734
1.0294430224145406,0.312094574280478
1.0588859836045912,0.3112922219486455
1.122725071256376,0.3095905107727923
1.1823336507104565,0.3080463768453499
1.2407729464566284,0.30657234343124495
1.3041654074744837,0.30501568082266334
1.3633273602946345,0.303600656920991
1.4274424783864688,0.30210627658188405
1.4903883127703945,0.30067681426002596
1.549103638956616,0.29937547736837855
1.6127721304145206,0.2979977246390743
1.672210113674721,0.29674146347008645
1.7304788132270128,0.2955367782502466
1.7937006780509879,0.2942585074745922
1.8526920346772586,0.29309171306167947
1.9166365565752128,0.29185406198508146
1.9794117947652585,0.29066536678691024
2.0379565247576,0.28957935150795977
2.101454420021624,0.2884251267681377
2.160721807087944,0.28736919577636916
2.2249423594259476,0.28624746200120293
2.2879936280560424,0.2851680141301427
2.3468143884884327,0.2841798189783042
2.4105883141925064,0.28312821147847544
2.4701317316988756,0.2821643226167758
2.5285058654973365,0.2812356311408256
2.591833164567481,0.28024575292287796
2.6509299554399206,0.27933800205386045
2.714979911584044,0.27837103809659086
2.7778605840202584,0.27743824639499287
2.836510748258769,0.2765824961550667
2.9001140777689622,0.2756695734134527
2.9594868990814516,0.27483112290268996
3.017690436686032,0.27402169060716297
3.0808471395622963,0.27315697414969653
3.139773334240856,0.27236257281796905
3.2036526941910988,0.2715145345556902
3.263301545943637,0.2707346356161353
3.3217811139882674,0.26998094327704203
3.385213847304581,0.2691753143351686
3.44441607242319,0.2684342773006821
3.5085714628134825,0.2676427615378315
3.5715575694958663,0.26687701532787317
3.630313167980546,0.2661725646109426
3.694021931736909,0.26541920558158405
3.753500187295568,0.26472546319602364
3.8118091591463177,0.26405412486393964
3.875071296268751,0.26333533310677165
3.93410292519348,0.2626733785865862
3.935132566030699,0.2626619065347868
3.936162206867918,0.26265043699554574
3.9382214885423563,0.2626275054505895
3.9423400518912333,0.26258167246583686
3.950577178588987,0.2624901266859525
3.967051431984495,0.26230751404494096
3.968081072821714,0.26229611619890497
3.9691107136589334,0.2622847322040231
3.971169995333372,0.2622619602780153
3.975288558682249,0.2622164461382847
3.9835256853800027,0.262125536481399
3.984555326217222,0.26211418387547625
3.985584967054441,0.2621028337331285
3.9876442487288797,0.26208014083513087
3.9917628120777566,0.2620347845578307
3.992792452914976,0.26202345163238405
3.993822093752195,0.26201212116248546
3.9958813754266336,0.2619894675853317
3.996911016263853,0.26197814447607726
3.997940657101072,0.26196682381837505
3.998970297938291,0.2619555056112201
3.99999993877551,0.261944189853622


==> signaling_1.tex <==
1.0000000612244897,0.32218535509759577
1.0009201537616788,0.322192439988913
1.001840246298868,0.32219952278787173
1.0036804313732461,0.3222136821135254
1.0073608015220024,0.32224197570934776
1.0147215418195152,0.3222984629468023
1.0294430224145406,0.32241103973316687
1.0588859836045912,0.32263461935939175
1.122725071256376,0.32311234023496704
1.1823336507104565,0.3235499550389539
1.2407729464566284,0.3239713464888614
1.3041654074744837,0.324420199193933
1.3633273602946345,0.32483161223032364
1.4274424783864688,0.32526959156970303
1.4903883127703945,0.325691881503634
1.549103638956616,0.32607913957933315
1.6127721304145206,0.32649204867525783
1.672210113674721,0.3268711390440543
1.7304788132270128,0.32723697422346365
1.7937006780509879,0.32762761191746115
1.8526920346772586,0.3279863771083615
1.9166365565752128,0.3283692041882244
1.9794117947652585,0.32873907966924415
2.0379565247576,0.3290788706495433
2.101454420021624,0.3294419437376164
2.160721807087944,0.3297758383137197
2.2249423594259476,0.33013235368610205
2.2879936280560424,0.3304771801293132
2.3468143884884327,0.33079435399092827
2.4105883141925064,0.3311334438686402
2.4701317316988756,0.3314456564758501
2.5285058654973365,0.3317477345810275
2.591833164567481,0.3320710756822046
2.6509299554399206,0.33236881741361285
2.714979911584044,0.3326872653098393
2.7778605840202584,0.3329957078148423
2.836510748258769,0.33327974768923496
2.9001140777689622,0.33358388933738203
2.9594868990814516,0.33386423825083733
3.017690436686032,0.33413580413670735
3.0808471395622963,0.33442691090206134
3.139773334240856,0.33469524355809266
3.2036526941910988,0.3349826430504297
3.263301545943637,0.3352478058327502
3.3217811139882674,0.33550483385478713
3.385213847304581,0.33578041593090296
3.44441607242319,0.3360346643120495
3.5085714628134825,0.3363070346979408
3.5715575694958663,0.3365713227413469
3.630313167980546,0.3368151340349217
3.694021931736909,0.33707658867856427
3.753500187295568,0.3373180047384682
3.8118091591463177,0.3375522162915455
3.875071296268751,0.33780362539789194
3.93410292519348,0.33803573960644145
3.935132566030699,0.33803976720681733
3.936162206867918,0.3380437940926692
3.9382214885423563,0.33805184572175606
3.9423400518912333,0.3380679404161874
3.950577178588987,0.3381000956037259
3.967051431984495,0.33816426960106555
3.968081072821714,0.33816827445518166
3.9691107136589334,0.33817227860240134
3.971169995333372,0.33818028477709156
3.975288558682249,0.338196288654094
3.9835256853800027,0.33822826257137245
3.984555326217222,0.33823225614342695
3.985584967054441,0.33823624901235216
3.9876442487288797,0.3382442326417509
3.9917628120777566,0.33826019147330916
3.992792452914976,0.3382641794268879
3.993822093752195,0.33826816667921056
3.9958813754266336,0.338276139081021
3.996911016263853,0.3382801242309757
3.997940657101072,0.33828410868060677
3.998970297938291,0.3382880924301484
3.99999993877551,0.3382920754798332


==> signaling_2.tex <==
1.0000000612244897,0.32218535353623357
1.0009201537616788,0.3221689773975947
1.001840246298868,0.3221526059982741
1.0036804313732461,0.3221198774068128
1.0073608015220024,0.32205447697732603
1.0147215418195152,0.32192390253187464
1.0294430224145406,0.3216636545239008
1.0588859836045912,0.3211467243561387
1.122725071256376,0.3200418792664281
1.1823336507104565,0.31902940090340337
1.2407729464566284,0.31805410601722184
1.3041654074744837,0.31701487342271667
1.3633273602946345,0.3160619807730623
1.4274424783864688,0.3150471941497265
1.4903883127703945,0.3140684049775512
1.549103638956616,0.3131705068017526
1.6127721304145206,0.3122128108498814
1.672210113674721,0.31133325954385943
1.7304788132270128,0.31048419519973947
1.7937006780509879,0.30957727676101604
1.8526920346772586,0.3087440904161899
1.9166365565752128,0.3078547440523212
1.9794117947652585,0.30699521131745167
2.0379565247576,0.30620535244677966
2.101454420021624,0.3053611213669563
2.160721807087944,0.30458450726075637
2.2249423594259476,0.303755035333905
2.2879936280560424,0.30295251946060514
2.3468143884884327,0.3022141513797896
2.4105883141925064,0.30142454284665254
2.4701317316988756,0.3006973190329097
2.5285058654973365,0.29999351658133283
2.591833164567481,0.2992399728657007
2.6509299554399206,0.2985459040486305
2.714979911584044,0.2978033712168958
2.7778605840202584,0.29708397522027125
2.836510748258769,0.2964213265945936
2.9001140777689622,0.2957116028261426
2.9594868990814516,0.29505723614578067
3.017690436686032,0.294423219945609
3.0808471395622963,0.2937434180828763
3.139773334240856,0.29311664844632596
3.2036526941910988,0.29244518224737276
3.263301545943637,0.2918255215757707
3.3217811139882674,0.2912247360921984
3.385213847304581,0.29058043403507583
3.44441607242319,0.28998587377811263
3.5085714628134825,0.2893487905829309
3.5715575694958663,0.28873046915324824
3.630313167980546,0.2881599295134837
3.694021931736909,0.28754796941316485
3.753500187295568,0.28698278881106465
3.8118091591463177,0.28643436199526645
3.875071296268751,0.2858455419690515
3.93410292519348,0.28530179838507486
3.935132566030699,0.2852923624884037
3.936162206867918,0.28528292823283585
3.9382214885423563,0.28526406464282933
3.9423400518912333,0.28522635713206834
3.950577178588987,0.2851510206656933
3.967051431984495,0.28500066098224086
3.968081072821714,0.28499127733157714
3.9691107136589334,0.28498189530469054
3.971169995333372,0.28496313612009705
3.975288558682249,0.28492563721261144
3.9835256853800027,0.2848507171244963
3.984555326217222,0.2848413593899521
3.985584967054441,0.284832003270622
3.9876442487288797,0.2848132958754782
3.9917628120777566,0.2847759004443402
3.992792452914976,0.2847665556166099
3.993822093752195,0.28475721239984036
3.9958813754266336,0.2847385307970543
3.996911016263853,0.28472919240997946
3.997940657101072,0.2847198556317432
3.998970297938291,0.28471052046181305
3.99999993877551,0.2847011868996648

